Multiparty Session Types for Safe Runtime Adaptation in an Actor Language (Extended version)

Human fallibility, unpredictable operating environments, and the heterogeneity of hardware devices are driving the need for software to be able to adapt as seen in the Internet of Things or telecommunication networks. Unfortunately, mainstream programming languages do not readily allow a software component to sense and respond to its operating environment, by discovering, replacing, and communicating with components that are not part of the original system design, while maintaining static correctness guarantees. In particular, if a new component is discovered at runtime, there is no guarantee that its communication behaviour is compatible with existing components. We address this problem by using multiparty session types with explicit connection actions, a type formalism used to model distributed communication protocols. By associating session types with software components, the discovery process can check protocol compatibility and, when required, correctly replace components without jeapordising safety. We present the design and implementation of EnsembleS, the first actor-based language with adaptive features and a static session type system, and apply it to a case study based on an adaptive DNS server. We formalise the type system of EnsembleS and prove the safety of well-typed programs, making essential use of recent advances in non-classical multiparty session types.

==> figures/ensemble-dns-session.tex <==
\begin{wrapfigure}{l}{0.525\textwidth}
%\setlength{\columnsep}{\colsep}
% , multicols=2]
\begin{lstlisting}[ escapechar=@,language=ensemble]
type Client is session(
  connect RootServer;
  RootRequest(DomainName) to RootServer;
  choice at RootServer{
    TLDResponse(ZoneServerAddress) from RootServer;
    disconnect RootServer;
    rec Lookup {
      connect ZoneServer;
      ResolutionRequest(DomainName) to ZoneServer;
      choice at ZoneServer {
        PartialResolution(ZoneServerAddress)
          from ZoneServer;
        disconnect ZoneServer;
        continue Lookup;
      } or {
        InvalidDomain(String) from ZoneServer;
        disconnect ZoneServer;
      } or {
        ResolutionComplete(IPAddress) from ZoneServer;
        disconnect ZoneServer;
      }
    }
  } or {
    InvalidTLD(String) from RootServer;
    disconnect RootServer;
  }
)
\end{lstlisting}
\caption{EnsembleS DNS client \texttt{session} type \vspace{-1em}}
\label{lst:ensemble-dns-client-session}
\end{wrapfigure}


==> figures/ensemble-dns.tex <==
\begin{figure}[t]
\setlength{\columnsep}{\colsep}
%\setlength{\columnsep}{30pt}
  \begin{lstlisting}[ escapechar=@,
  language=ensemble,
  %float=tp,
  %caption={EnsembleS Client},
  basicstyle=\ttfamily\scriptsize,
  numbers={left}, multicols=2]
type Iclient is interface(
	out{RootServer,string} RootServer_stringOut,
	in {RootServer,string} RootServer_stringIn,
	out{ZoneServer,string} ZoneServer_stringOut,
	in {ZoneServer,string} ZoneServer_stringIn,
	in {ZoneServer,choice_enum}	ZoneServer_choiceIn,
	in {RootServer,choice_enum}	RootServer_choiceIn)

type choice_enum is
	enum(TLDResponse,PartialResolution,
	InvalidDomain,ResolutionComplete,
	InvalidTLD)

query find_name(string n){ $name == n; }

actor c presents Iclient
	follows Client {
	dom_name = "nii.ac.jp";
	constructor() { }
	behaviour{
		rootQuery = find_name("jp");
		// Find Root Server
		root_s =
			discover(IServer, RootServer, rootQuery);
		// search until root_s non-empty
		link me with root_s[0];
		send domain_name on RootServer_stringOut;
		receive c_msg	from RootServer_choiceIn;
		switch(c_msg){
			case TLDResponse:
				receive ZoneServerAddr_msg
					from RootServer_stringIn;
			unlink RootServer;
while(true) Lookup : {
	// Find ZoneServer
	zone_s =
    discover(IServer,	ZoneServer,
      find_name(ZoneServerAddr_msg));
	link me with zone_s[0];
	// Ask ZoneServer
	send dom_name on ZoneServer_stringOut;
	receive c_msg2 from ZoneServer_choiceIn;
	switch(c_msg2){
		case PartialResolution:
			receive str_msg from ZoneServer_stringIn;
			ZoneServerAddr_msg := str_msg;
			unlink ZoneServer;
			continue Lookup;
		case InvalidDomain:
			receive str_msg from ZoneServer_stringIn;
			unlink ZoneServer;
			break;
		case ResolutionComplete:
			receive str_msg from ZoneServer_stringIn;
			unlink ZoneServer;
			break Lookup;
		}
		// keep looking
	}
case InvalidTLD:
	 receive str_msg from RootServer_stringIn;
	 unlink RootServer;
} } }
  \end{lstlisting}
\caption{EnsembleS DNS client}
\label{lst:ensemble-dns-client}
\end{figure}




==> figures/operational-semantics.tex <==
\begin{figure*}
  \begin{minipage}{0.45\textwidth}
  {\small
~\totheleft{Runtime syntax}
    \[
  \begin{array}{lccl}
    %\text{Names} & a, b, c \\
    \text{Session names} & s \\
    \text{Names} & \alpha & ::= & a \midspace s \\
    \text{Values} & V, W & ::= & \cdots \midspace a \\
    \text{Connection state} & \sigma & ::= & \bot \midspace \connsess{s}{\theta} \\
    \text{Connection environments} & \theta & ::= & \cdot \midspace \theta, \role{r} \mapsto a \\
    \text{Runtime types} & R & ::= &  \\
    \text{Runtime environments} \!\! & \Delta & ::= &
      \cdot \midspace \Delta, a : \rtproc{\tyindex{G}{r}}{S} \midspace s : G \\
\text{Evaluation contexts} & E & ::= & [~] \mid \efflet{x}{E}{M} \\
  \text{Configurations} & \config{C}, \config{D}, \config{E} & ::= & (\nu \alpha)
  \config{C} \midspace \config{C} \parallel \config{D} \midspace \eactor{a}{M}{\sigma}{\kappa}
  \end{array}
\]
}
  \end{minipage}
  \hspace{4em}
  \begin{minipage}{0.4\textwidth}
{\small
~Reduction rules for terms \hfill \framebox{$M \teval M'$}
    \[
    \begin{array}{rcl}
        \efflet{x}{\effreturn{V}}{M} & \teval & M \{ V / x \} \\
        l : M & \teval & M \{ l : M / \continue{l} \} \\
        E[M] & \teval & E[M'] \quad \text{ if } M \teval M'
    \end{array}
\]
}
\end{minipage}

{\small
~Equivalence \hfill \framebox{$\config{C} \equiv \config{C'}$}
  \begin{mathpar}
    \config{C} \parallel \config{D} \equiv \config{D} \parallel \config{C}

    \config{C} \parallel (\config{D} \parallel \config{E}) \equiv
    (\config{C} \parallel \config{D}) \parallel \config{E}

    (\nu \alpha_1)(\nu \alpha_2)\config{C} \equiv (\nu \alpha_2)(\nu \alpha_1)\config{C}

    \config{C} \parallel (\nu \alpha) \config{D} \equiv (\nu \alpha) (\config{C} \parallel \config{D}) \quad
    \text{if } \alpha \not\in \textsf{fn}(\config{C})

    (\nu \alpha) \config{C} \equiv \config{C} \quad \text{if } \alpha \not\in \textsf{fn}(\config{C})
  \end{mathpar}
}
%
{\small
~Reduction rules for configurations \hfill \framebox{$\config{C} \ceval \config{C'}$}
\begin{mathpar}
  \inferrule
  [E-LinkInit]
  {
    s \text{ fresh} \\
    \role{s} \not\in \theta_1 \\ \role{r} \not\in \theta_2 \\\\
    a.\mkwd{sessionType} = \tyindex{G}{\role{r}} \\
    b.\mkwd{sessionType} = \tyindex{G}{\role{s}} \\
  }
  { \eactor{a}{E[\link{b}{M}]}{\bot}{\kappa_1} \!\parallel\!
    \eactor{b}{E'[\accept{\role{r}}]}{\bot}{\kappa_2} \! \ceval \\\\
    (\nu s) (\eactor{a}{E[\effreturn{()}]}{\connsess{s}{\role{s} \!\mapsto\! b}}{\kappa_1}
    \!\parallel\!
    \eactor{b}{E'[\effreturn{()}]}{\connsess{s}{\role{r} \!\mapsto\! a}}{\kappa_2})
  }

  \inferrule
  [E-Link]
  {
    \role{s} \not\in \theta_1 \\ \role{r} \not\in \theta_2 \\
    a.\mkwd{sessionType} = \tyindex{G}{\role{r}} \\
    b.\mkwd{sessionType} = \tyindex{G}{\role{s}} \\
  }
  { \eactor{a}{E[\link{b}{M}]}{\connsess{s}{\theta_1}}{\kappa_1} \!\parallel\! \eactor{b}{E'[\accept{\role{r}}]}{\bot}{\kappa_2} \! \ceval \\\\
    \eactor{a}{E[\effreturn{()}]}{\connsess{s}{\theta_1[\role{s} \!\mapsto\! b]}}{\kappa_1}
    \!\parallel\!
    \eactor{b}{E'[\effreturn{()}]}{\connsess{s}{\theta_2[\role{r} \!\mapsto\! a]}}{\kappa_2}
  }

  \inferrule
  [E-LinkFail]
  { }
  { \eactor{a}{E[\link{b}{M}]}{\sigma_1}{\kappa_1} \parallel \eactor{b}{\effreturn{V}}{\bot}{\bstop}
    \ceval \\\\
    \eactor{a}{E[M]}{\sigma_1}{\kappa_1} \parallel \eactor{b}{\effreturn{V}}{\bot}{\bstop}
  }

  \inferrule
  [E-Unlink]
  { }
  { \eactor{a}{E[\unlink{\role{s}}]}{\connsess{s}{\theta_1[\role{s} \!\mapsto\! b]}}{\kappa_1} \parallel
    \eactor{b}{E'[\unlink{\role{r}}]}{\connsess{s}{\theta_2[\role{r} \!\mapsto\! a]}}{\kappa_2} \!\ceval \\\\
    \eactor{a}{E[\effreturn{()}]}{\connsess{s}{\theta_1}}{\kappa_1} \parallel
    \eactor{b}{E'[\effreturn{()}]}{\connsess{s}{\theta_2}}{\kappa_2}
  }

  \inferrule
  [E-Comm]
  { (\role{r} \mapsto b) \in \theta_1 \\ (\role{s} \mapsto a) \in \theta_2 }
  {
    \eactor{a}{E[\send{V}{\cout{\role{r}}{U}}]}{\connsess{s}{\theta_1}}{\kappa_1}
    \parallel \eactor{b}{E'[\recv{\cin{\role{s}}{U}}]}{\connsess{s}{\theta_2}}{\kappa_2} \!\ceval \\\\
    \eactor{a}{E[\effreturn{()}]}{\connsess{s}{\theta_1}}{\kappa_1} \parallel
    \eactor{b}{E'[\effreturn{V}]}{\connsess{s}{\theta_2}}{\kappa_2}
  }

  \inferrule
  [E-Branch]
  { j \in I }
  {
    \eactor{a}{E[\select{\role{r}}{\ell_j}]}{\connsess{s}{\theta_1}}{\kappa_1}
  \parallel \eactor{b}{E'[\offer{\role{r}}{\{\ell_i : M_i \}_{i \in I}}]}{\connsess{s}{\theta_2}}{\kappa_2} \!\ceval \\\\
    \eactor{a}{E[\effreturn{()}]}{\connsess{s}{\theta_1}}{\kappa_1} \parallel
    \eactor{b}{E'[M_j]}{\connsess{s}{\theta_2}}{\kappa_2}
  }

  \inferrule
  [E-Leave]
  { }
  { \eactor{a}{\effreturn{V}}{\connsess{s}{\cdot}}{M} \ceval \eactor{a}{M}{\bot}{M} }


  \inferrule
  [E-Loop]
  { }
  { \eactor{a}{\effreturn{V}}{\bot}{M} \ceval \eactor{a}{M}{\bot}{M} }

  \inferrule
  [E-New]
  { b \text{ is fresh} \\ u.\mkwd{behaviour} = M }
  {
    \eactor{a}{E[\new{u}]}{\sigma}{\kappa} \ceval \\\\
    (\nu b) (\eactor{a}{E[\effreturn{b}]}{\sigma}{\kappa} \parallel
   \eactor{b}{M}{\bot}{M})
  }

  \inferrule
  [E-Replace]
  { }
  { \eactor{a}{E[\replace{\kappa'}{b}]}{\sigma_1}{\kappa_1} \parallel
    \eactor{b}{N}{\sigma_2}{\kappa_2} \ceval \\\\
    \eactor{a}{E[\effreturn{()}]}{\sigma_1}{\kappa_1} \parallel
    \eactor{b}{N}{\sigma_2}{\kappa'} }

  \inferrule
  [E-ReplaceSelf]
  { }
  { \eactor{a}{E[\replace{\kappa'}{a}]}{\sigma}{\kappa}
    \ceval \\\\
  \eactor{a}{E[\effreturn{()}]}{\sigma}{\kappa'}}

  \inferrule
  [E-Discover]
  { b.\mkwd{sessionType} = \tyindex{G}{r} \\
    \neg (M = V \wedge \kappa_2 = \bstop) \\
    \matches{b}{q} }
  { \eactor{a}{E[\discover{G}{\role{r}}{q}]}{\sigma_1}{\kappa_1} \parallel
    \eactor{b}{M}{\sigma_2}{\kappa_2} \ceval
    \eactor{a}{E[\effreturn{b}]}{\sigma_1}{\kappa_1} \parallel
    \eactor{b}{M}{\sigma_2}{\kappa_2}
  }

  \inferrule
  [E-Self]
  { }
  { \eactor{a}{E[\self]}{\sigma}{\kappa} \ceval \eactor{a}{E[\effreturn{a}]}{\sigma}{\kappa} }

\inferrule
   [E-LiftM]
   { M \teval M' }
   {
     \eactor{a}{E[M]}{\sigma}{\kappa} \ceval
     \eactor{a}{E[M']}{\sigma}{\kappa}
   }

  \inferrule
  [E-Equiv]
  { \config{C} \equiv \config{C}' \\
    \config{C}' \ceval \config{D}' \\
    \config{D}' \equiv \config{D} }
  { \config{C} \ceval \config{D} }

   \inferrule
   [E-Par]
   { \config{C} \ceval \config{C}' }
   { \config{C} \parallel \config{D} \ceval \config{C}' \parallel \config{D} }

   \inferrule
   [E-Nu]
   { \config{C} \ceval \config{D} }
   { (\nu a) \config{C} \ceval (\nu a) \config{D}}
\end{mathpar}
 }
\caption{Runtime syntax, equivalence and reduction rules for terms and configurations}
\label{fig:semantics-def}
\end{figure*}%




==> figures/static-typing.tex <==
\begin{figure*}
{
  \small

  \begin{minipage}[t]{0.3\textwidth}
Typing rules for definitions \hfill \framebox{$ \vdash P$}
  \begin{mathpar}
    \inferrule
    { \project{G}{\role{r}} = S \\
      \cdot \midspace S \triangleright M : A \triangleleft \localend
    }
    { \vdash \actordef{u}{G}{\role{r}}{M}  }
  \end{mathpar}
\end{minipage}
\quad
\begin{minipage}[t]{0.4\textwidth}
~Typing rules for behaviours \hfill \framebox{$\jarg{\tyindex{G}{r}} \Gamma \vdash \kappa$}
  \begin{mathpar}
    \inferrule
    { }
    { \jarg{\tyindex{G}{\role{r}}} \Gamma \vdash \bstop }

    \inferrule
    { \project{G}{\role{r}} = S \\\\
      \jarg{\tyindex{G}{\role{r}}} \Gamma \midspace S \triangleright M : A \triangleleft \localend }
    { \jarg{\tyindex{G}{\role{r}}} \Gamma \vdash M }
  \end{mathpar}
\end{minipage}
\quad
\begin{minipage}[t]{0.25\textwidth}
Typing rules for values\hfill \framebox{$\Gamma \vdash V : A$}
\begin{mathpar}
\inferrule
  [T-Name]
  { a : A \in \Gamma }
  { \Gamma \vdash a : A }

  \inferrule
  [T-Unit]
  { }
  { \Gamma \vdash () : \one }
\end{mathpar}
\end{minipage}

~Typing rules for computations\hfill \framebox{$\jarg{\tyindex{G}{r}} \Gamma \midspace S \triangleright M : A \triangleleft S' $}
\begin{mathpar}
\inferrule
  [T-Let]
  { \jarg{\tyindex{G}{r}} \Gamma \midspace S \triangleright M : A \triangleleft S' \\\\
    \jarg{\tyindex{G}{r}} \Gamma, x : A \midspace S' \triangleright N : B \triangleleft S'' }
  { \jarg{\tyindex{G}{r}} \Gamma \midspace S \triangleright \efflet{x}{M}{N} : B \triangleleft S'' }

\inferrule
  [T-Return]
  { \Gamma \vdash V : A }
  { \jarg{\tyindex{G}{r}} \Gamma \midspace S \triangleright \effreturn{V} : A \triangleleft S }

\inferrule
  [T-Rec]
  { \jarg{\tyindex{G}{r}} \Gamma, l : S \midspace S \triangleright M : A \triangleleft S }
  { \jarg{\tyindex{G}{r}} \Gamma \midspace S \triangleright (\annst{l}{M}) : A \triangleleft  S }

\inferrule
  [T-Continue]
  { }
  { \jarg{\tyindex{G}{r}} \Gamma, l : S \midspace S \triangleright \continue{l} : A \triangleleft S'  }

\inferrule
  [T-New]
  { u.\mkwd{sessionType} = \tyindex{G'}{s} }
  { \jarg{\tyindex{G}{r}} \Gamma \midspace S \triangleright \new{u} : \pid{G'}{\role{s}} \triangleleft S }

  \inferrule
  [T-Link]
  { \Gamma \vdash V : \pid{G}{\role{s}} \\
    \Gamma \midspace \localconn{\role{s}}{S} \triangleright M : \one \triangleleft S }
  { \jarg{\tyindex{G}{r}} \Gamma \midspace \localconn{\role{s}}{S} \triangleright \link{V}{M} : \one \triangleleft S }

  \inferrule
  [T-Accept]
  { }
  { \jarg{\tyindex{G}{r}} \Gamma \midspace \localaccept{\role{s}}{S} \triangleright \accept{\role{s}} : \one \triangleleft S }

  \inferrule
  [T-Unlink]
  { }
  { \jarg{\tyindex{G}{r}} \Gamma \midspace \localdisconn{\role{s}}{S} \triangleright \unlink{\role{s}} : \one \triangleleft S }

\inferrule
  [T-Send]
  { \Gamma \vdash V : U }
  { \jarg{\tyindex{G}{r}} \Gamma \midspace \localsend{\role{s}}{U}{S} \triangleright \send{V}{\cout{\role{s}}{U}} : \one \triangleleft S }

\inferrule
  [T-Receive]
  { }
  { \jarg{\tyindex{G}{r}} \Gamma \midspace \localrecv{\role{s}}{U}{S} \triangleright
    \recv{\cin{\role{s}}{U}} : U \triangleleft S }

\inferrule
  [T-Select]
  { j \in I }
  {
  \jarg{\tyindex{G}{r}} \Gamma \midspace \localselect{\role{s}}{\ell_i : S_i}_{i \in I}  \triangleright
    \select{\role{s}}{\ell_j} : \one \triangleleft S_j
  }

  \inferrule
  [T-Offer]
  { (\jarg{\tyindex{G}{r}} \Gamma \midspace S_i \triangleright M_i : A \triangleright S)_i }
  {
    \jarg{\tyindex{G}{r}} \Gamma \midspace \localoffer{\role{s}}{\ell_i : S_i}_{i \in I} \triangleright
    \offer{\role{s}}{\{ \ell_i : M_i \}_i} : A \triangleleft S
  }

% \inferrule
%   [T-Switch]
%   { \Gamma \vdash V : \enumty{E} \\
%     (\jarg{\tyindex{G}{r}} \Gamma \midspace S_i \triangleright M_i : A \triangleleft S' )_i }
%   { \jarg{\tyindex{G}{r}} \Gamma \midspace \tsenum{\{ \ell_i : S_i\}_{i \in
%   \enumty{E}}} \triangleright
%   \switch{V}{\ell_i : M_i}_{i \in \enumty{E}} : A \triangleleft S' }

  \inferrule
  [T-Discover]
  { }
  { \jarg{\role{r}} \Gamma \midspace S \triangleright \discover{G}{\role{r}}{q} : \pid{G}{\role{r}} \triangleleft S}

  \inferrule
  [T-Replace]
  { \jarg{\tyindex{G'}{\role{s}}} \Gamma \vdash \kappa \\ \Gamma \vdash V : \pid{G'}{\role{s}} }
  { \jarg{\tyindex{G}{r}} \Gamma \midspace S \triangleright \replace{\kappa}{V} : \one\triangleleft S }

  \inferrule
  [T-Self]
  { }
  { \jarg{\tyindex{G}{r}}  \Gamma \midspace S \triangleright \self : \pid{G}{\role{r}} \triangleleft S }
\end{mathpar}
}
\caption{Typing rules for definitions, behaviours, values and computations}
\label{fig:ensemble-typing}
\end{figure*}

